Combating Reinforcement Learning's Sisyphean Curse with Intrinsic Fear

Many practical environments contain catastrophic states that an optimal agent would visit infrequently or never. Even on toy problems, Deep Reinforcement Learning (DRL) agents tend to periodically revisit these states upon forgetting their existence under a new policy. We introduce intrinsic fear (IF), a learned reward shaping that guards DRL agents against periodic catastrophes. IF agents possess a fear model trained to predict the probability of imminent catastrophe. This score is then used to penalize the Q-learning objective. Our theoretical analysis bounds the reduction in average return due to learning on the perturbed objective. We also prove robustness to classification errors. As a bonus, IF models tend to learn faster, owing to reward shaping. Experiments demonstrate that intrinsic-fear DQNs solve otherwise pathological environments and improve on several Atari games.

==> analysis.tex <==
\appendix
\section{Loss in Optimal Value (Proof of Theorem~\ref{thm:ideal})} \label{sec:proof-T1}
The average return of the reward under a policy $\pi$ is as follows:
\begin{align}\label{eq:eta}
\eta_M(\pi) = \lim_{T\rightarrow \infty}\frac{1}{T}\mathbb{E}\left[\sum_t^T r_t|\pi\right]\,.
\end{align}
Let us assume that any stationary policy $\pi$ induces a stationary distribution $\omega_\pi(s),~ s\in\SSS$. Therefore we can rewrite Eq.~\ref{eq:eta} in terms of stationary distribution \cite{puterman2014markov}.
\begin{align*}
\eta_M(\pi) = \lim_{T\rightarrow \infty} \frac{1}{T} \mathbb{E}\left[\sum_t r_t|\pi\right] = \sum_{s\in\SSS}\sum_{a\in\AAA}\omega_\pi(s)\pi(a|s)\RRR(s,a)\,.
\end{align*}
In RL, we are interested in a policy $\pi^*$ that maximizes the expected average reward:
\begin{align*}
\pi^* := \arg\max_{\pi}\eta_M(\pi)\,.
\end{align*}
Denote $\eta_M^* = \eta_M(\pi^*)$. 
In a first place, the optimization in Eq.~\ref{eq:eta} looks linear in $\pi$ but actually the policy $\pi$ derives the stationary distribution $\omega_\pi(\cdot)$, which makes the optimization problem harder.

Given the policy $\pi$, let's define the joint distribution in $(s,a)$ as follows:
\begin{align*}
\mu_{\pi}(s,a):= \mathbb{P}(s,a|\pi)=\omega_\pi(s)\pi(a|s),~\forall s\in\SSS,a\in\AAA\,.
\end{align*}
Then we can rewrite the optimization problem in terms of the joint probability distribution $\mu_{\pi}$.
\begin{align}
\eta_m(\mu_{\pi}):= \sum_{s\in\SSS}\sum_{a\in\AAA}\mu_{\pi}(s,a)\RRR(s,a)\,.
\end{align}
We can see that this new formalization, turns our optimization objective into a linear function of $\mu_{\pi}$. Since $\mu_{\pi}$ is a join distribution of $(s,a)$ under the model dynamics $\mathcal{T}$, it can not take any arbitrary value. Let $\Delta$ denote the set of feasible value for $\mu_{\pi}$, then
\begin{align}
\Delta:=\lbrace \mu : \mu \ge 0, \sum_{s,a} \mu(s,a) = 1, \sum_{a'}\mu(s',a') = \sum_{s,a}\mathcal{T}(s'|s,a)\mu(s,a), \forall s'\in\SSS\rbrace\,.
\end{align}
%Since $\sum_{s,a}\mu_{\pi}(s,a) = 1$ therefore 
Clearly, $\Delta$ is a polytope on the simplex in $\mathbb{R}^{S\times A}$.

Now, we can rewrite the optimization problem Eq.~\ref{eq:eta} as a constrained linear program on $\mu_{\pi}$:
\begin{align*}
\eta_M^* = \max_{\mu\in\Delta}\sum_{s\in\SSS}\sum_{a\in\AAA}\mu(s,a)\RRR(s,a)\,.
\end{align*}
This change of variable allows us to analyze the introduction of intrinsic fear in different situations. Among all the optimal policies of Eq.~\ref{eq:eta}, consider the one which minimizes $\epsilon:=\sum_{s\in\mathcal{C},a}\mu_{\pi^*}(s,a)$.
% $(i)-$ If the probability that at any time step the optimal agent happens to be in the danger zone, $\sum_{s\in\mathcal{C},a}\mu_{\pi^*}(s,a)$, is zero, and the intrinsic fear reward assigned to the states in this zone $\mathcal{C}$ is negative, then optimal policy in the original environment (without intrinsic reward) is the same as the optimal policy in the model with intrinsic reward. Moreover, the long term average reward provided under these models are same. (The intrinsic fear helps to learn the optimal behavior faster in the RL framework).

%$(ii)-$ Now, we consider the situation where the $\sum_{s\in\mathcal{C},a}\mu_{\pi^*}(s,a)$ is nonzero, but less than $\epsilon$.
let's assume that the negative reward assigned to the states in the danger zone is $\lambda(\RRR_{\max}-\RRR_{\min})$ and the optimal policy $\tilde{\pi}$ of the environment with the intrinsic fear has return of $\eta_{M,F}(\tilde{\pi})$.

Applying policy $\pi^*$ on the environment with intrinsic fear gives a return of $\eta_M^*-\lambda\epsilon(\RRR_{\max}-\RRR_{\min})$. Therefore, the return of $\tilde{\pi}$ on the environment with intrinsic fear, $\eta_{M,F}$, is lower bounded by  $\eta_M^*-\lambda\epsilon(\RRR_{\max}-\RRR_{\min})$. Therefore, applying $\tilde{\pi}$ on the environment without intrinsic fear gives a return of $\eta_{M}(\tilde{\pi})$ which is lower bounded by $\eta_M^*-\lambda\epsilon(\RRR_{\max}-\RRR_{\min})$.
\begin{align}
\eta_M^*\geq\eta_{M}(\tilde{\pi}) \geq \eta_{M,F}(\tilde{\pi})\geq \eta_M^*-\lambda\epsilon(\RRR_{\max}-\RRR_{\min}).
\end{align}
% If there exists a cost $\lambda$ such that the $\sum_{s\in\mathcal{C},a}\mu_{\tilde{\pi}}(s,a)$ under $\tilde{\pi}$ in either environments is negligible, since the set $\Delta$ is a convex polytope and $\RRR_{\min}\leq\RRR(s,a)\leq \RRR_{\max}$, then
% \begin{align}
% \eta_M^*\geq\eta_{M}(\tilde{\pi}) = \eta_M(\tilde{\pi})\geq \eta_M^*-\epsilon(\RRR_{\max}-\RRR_{\min}).
% \end{align}

% At the same time, the average return of the optimal policy $\pi^*$ on the environment with intrinsic fear, $\eta_{M,F}(\pi^*)$ is bounded as 
% \begin{align}
% \eta_{M,F}(\tilde{\pi})\geq\eta_{M,F}(\pi^*)\geq\eta_{M,F}(\tilde{\pi})-\lambda\epsilon(\RRR_{\max}-\RRR_{\min}).
% \end{align}


\subsection{Discounted Cumulative Reward}
For the $\gamma$-discounted setting, we are interested in 
\begin{align}
\eta(\pi) = (1-\gamma)\lim_{T\rightarrow \infty}\mathbb{E}\left[\sum_{t=0} \gamma^t r_t\right]
\end{align}
The above mentioned equations hold in this setting as well, $i.e.$, $\eta_M^*\geq\eta_{M}(\tilde{\pi}) \geq \eta_{M,F}(\tilde{\pi})\geq \eta_M^*-\lambda\epsilon(\RRR_{\max}-\RRR_{\min})$.



% Both of the above mentioned equations hold in this setting, $i.e.$, $\eta_M^*\geq\eta_{M,F}(\tilde{\pi}) = \eta_M(\tilde{\pi})\geq \eta_M^*-\epsilon(\RRR_{\max}-\RRR_{\min})$, and $\eta_{M,F}(\tilde{\pi})\geq\eta_{M,F}(\pi^*)\geq\eta_{M,F}(\tilde{\pi})-\lambda\epsilon(\RRR_{\max}-\RRR_{\min})$.




%##################################################################
\section{Imperfect Classifier (Proof of Theorem~\ref{thm:classifier})}\label{apx:concent}
In the previous section, we assumed that we have access to the perfect classifier $F$ which can exactly label the danger zone. This assumption does not hold in real world where we train the classifier. In this section we derive an analysis in order to show that imperfect classifier $\widehat{F}$ can not change the overall performance by much.

In general, in practical RL problems, we use discount factors $\gamma_{eval}<1$ \cite{kocsis2006bandit} in order to reduce the planing horizon, and computation cost. Moreover, \cite{jiang2015dependence} suggest that when we have an estimation (up to the confidence intervals) of our MDP model, it is better to use $\gamma \leq \gamma_{eval}$. They show that since larger discount factor enriches the class of optimal policies for a given set of plausible models, large discount factors enrich models and end up over fitting to the noisy estimate of the environment.

In this section, we show how to choose the discount factor $\gamma\leq\gamma_{eval}$ such that the learned Value function stays close to the Value function under the perfect classifier $F$ is perfect. Let, $V_{F_2,\gamma_2}^{\pi^*_{F_1,\gamma_{1}}}(s)$, $s\in\mathcal{S}$, denote the state value under the optimal policy of model with classifier $F_1$ under the discount factor $\gamma_1$ on the environment equipped with classifier $F$ and discount factor $\gamma_{2}$. On the same environment, $\omega_{F_2}^{\pi^*_{F_1,\gamma_{1}}}(s)$ denotes the stationary distribution over states.
We are interested in the average deviation on value functions caused by the imperfect classifier:
\begin{align*}
\mathcal{L}:=(1-\gamma_{eval})\sum_{s\in\mathcal{S}}\omega_{F}^{\pi^*_{\widehat{F},\gamma}}(s)
\left|V_{F,\gamma_{eval}}^{\pi^*_{F,\gamma_{eval}}}(s)-V_{F,\gamma_{eval}}^{\pi^*_{\widehat{F},\gamma}}(s)\right|
\end{align*}
This quantity can be upper bounded by 

\begin{align}\label{eq:loss}
\mathcal{L}\leq(1-\gamma_{eval})\|V_{F,\gamma_{eval}}^{\pi^*_{F,\gamma_{eval}}}-V_{F,\gamma_{eval}}^{\pi^*_{\widehat{F},\gamma}}\|_{\infty}
\end{align}
The goal is to find an $\gamma^*$ which minimizes this loss, i.e. $\gamma^*=\displaystyle argmin_{\gamma\leq\gamma_{eval}}\mathcal{L}$ with high probability. For simplicity and without loss of generality, let's assume that all the rewards, including the intrinsic fears, are in $[0,1]$ and call $\lambda'$, the transformed version of $\lambda$ \footnote{Shifting and then rescaling the reward is equivalent to shifting and rescaling the Q and Value function, and does not change the optimal policy. Moreover the mentioned transformation is $r\rightarrow (r-(\RRR_{min}-\lambda(\RRR_{\max}-\RRR_{\min})))/((\RRR_{\max}-\RRR_{\min})(1+\lambda))$, therefore, $\lambda'=\lambda/(1+\lambda)$}. One can decompose the upper bound in Eq.~\ref{eq:loss} as follows:
\begin{align}\label{eq:decomp}
V_{F,\gamma_{eval}}^{\pi^*_{F,\gamma_{eval}}}(s)-V_{F,\gamma_{eval}}^{\pi^*_{\widehat{F},\gamma}}(s)=
\left(V_{F,\gamma_{eval}}^{\pi^*_{F,\gamma_{eval}}}(s)-V_{F,\gamma}^{\pi^*_{F,\gamma_{eval}}}(s)\right)+\left(V_{F,\gamma}^{\pi^*_{F,\gamma_{eval}}}(s)-V_{F,\gamma_{eval}}^{\pi^*_{\widehat{F},\gamma}}(s)\right)
\end{align}
The first term is the deviation on value function when applying same policy on the same environment but with different discount factors. Since $\gamma\leq\gamma_{eval}$ we have $V_{F,\gamma}^{\pi^*_{F,\gamma_{eval}}}(s)\leq V_{F,\gamma_{eval}}^{\pi^*_{F,\gamma_{eval}}}(s)$.
\begin{align}\label{eq:firstpart}
V_{F,\gamma_{eval}}^{\pi^*_{F,\gamma_{eval}}}(s)-V_{F,\gamma}^{\pi^*_{F,\gamma_{eval}}}(s) &=\mathbb{E}_{F}\left[\sum_{t=0}^\infty \gamma_{eval}^tr_t|s_0 = s,\pi^*_{F,\gamma_{eval}}\right] - \mathbb{E}_{F}\left[\sum_{t=0}^\infty \gamma^tr_t|s_0 = s,\pi^*_{F,\gamma_{eval}}\right]\\
&=\mathbb{E}_{F}\left[\sum_{t=0}^\infty (\gamma^t_{eval}-\gamma^t)r_t|s_0 = s,\pi^*_{F,\gamma_{eval}}\right]\leq \left(\frac{1}{1-\gamma_{eval}}-\frac{1}{1-\gamma}\right)
\end{align}
The second part of Eq.~\ref{eq:decomp} is the deviation in value function under different policies and different classifiers. Again, since $\gamma\leq \gamma_{eval}$, we have $V_{F,\gamma_{eval}}^{\pi^*_{\widehat{F},\gamma}}(s)\geq V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)$
\begin{align}
V_{F,\gamma}^{\pi^*_{F,\gamma_{eval}}}(s)-V_{F,\gamma_{eval}}^{\pi^*_{\widehat{F},\gamma}}(s)\leq 
V_{F,\gamma}^{\pi^*_{F,\gamma_{eval}}}(s)-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)\leq
V_{F,\gamma}^{\pi^*_{F,\gamma}}(s)-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)
\end{align}
where the last inequality is due to the optimality of $\pi^*_{F,\gamma}$ on the environment of $F,\gamma$. To bound this part we exploit the proof trick used in \cite{jiang2015dependence}.
\begin{align}
V_{F,\gamma}^{\pi^*_{F,\gamma}}(s)-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s) =
\left(V_{F,\gamma}^{\pi^*_{F,\gamma}}(s)-V_{\widehat{F},\gamma}^{\pi^*_{F,\gamma}}(s)\right) +
\left(V_{\widehat{F},\gamma}^{\pi^*_{F,\gamma}}(s)-V_{\widehat{F},\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)\right)+
\left(V_{\widehat{F},\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)\right)
\end{align}
since the middle term is negative we have

\begin{align}\label{eq:absval}
V_{F,\gamma}^{\pi^*_{F,\gamma}}(s)-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s) \leq
\left(V_{F,\gamma}^{\pi^*_{F,\gamma}}(s)-V_{\widehat{F},\gamma}^{\pi^*_{F,\gamma}}(s)\right) +
\left(V_{\widehat{F},\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)\right)\leq 2\max_{\lbrace\pi^*_{\widehat{F},\gamma},\pi^*_{\widehat{F},\gamma}\rbrace}\left|V_{\widehat{F},\gamma}^{\pi}(s)-V_{F,\gamma}^{\pi}(s)\right|
\end{align}
This quantity $V_{\widehat{F},\gamma}^{\pi}(s)-V_{F,\gamma}^{\pi}(s)$ is the difference between the performance of the same policy on two different environments. These two values functions should satisfy the following bellman equations:
\begin{align*}
V_{{F},\gamma}^{\pi}(s) &= \mathcal{R}(s,\pi(s))+\lambda' F(s) + \gamma \sum_{s'\in\mathcal{S}}\mathcal{T}(s'|s,\pi(s))V_{{F},\gamma}^{\pi}(s')\\
V_{\widehat{F},\gamma}^{\pi}(s) &= \mathcal{R}(s,\pi(s))+\lambda'\widehat{F}(s) + \gamma \sum_{s'\in\mathcal{S}}\mathcal{T}(s'|s,\pi(s))V_{\widehat{F},\gamma}^{\pi}(s')
\end{align*}
To compute the solution two this equation, we use dynamic programing. Let initialize $V_0,\widehat{V} = V$(an arbitrary value) and construct the following updates.
\begin{align*}
\textit{for } i \in\lbrace 1,\ldots \infty\rbrace & \\
V^\pi_i(s) &= \mathcal{R}(s,\pi(s))+\lambda' F(s) + \gamma \sum_{s'\in\mathcal{S}}\mathcal{T}(s'|s,\pi(s))V^\pi_{i-1}(s)\\
\widehat{V}^\pi_i(s) &= \mathcal{R}(s,\pi(s))+\lambda'\widehat{F}(s) + \gamma \sum_{s'\in\mathcal{S}}\mathcal{T}(s'|s,\pi(s))\widehat{V}^\pi_{i-1}(s')
\end{align*}

As $i$ tends to infinity, these two dynamics updates converge to $V_{{F},\gamma}^{\pi}(s)$, and $V_{\widehat{F},\gamma}^{\pi}(s)$ respectively. To bound the right hand side of Eq.~\ref{eq:absval} we have
\begin{align}\label{eq:belman_update}
\begin{split}
V^\pi_i(s) - \widehat{V}^\pi_i(s) = \lambda'{F}(s) - \lambda'\widehat{F}(s) &+ \gamma \sum_{s'\in\mathcal{S}}\mathcal{T}(s'|s,\pi(s))\left({V}_{i-1}(s')-\widehat{V}_{i-1}(s')\right)\\
&\leq\lambda' \sum_{i'=0}^{i}\gamma^{i'}\max_{s}\left|{F}(s) - \widehat{F}(s)\right|
\end{split}
\end{align}
As $i$ tends to infinity, we have 

\begin{align*}
\left|V_{F,\gamma}^{\pi^*_{F,\gamma}}(s)-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}(s)\right| &= \max_{\pi}	\left|\lim_{i\rightarrow \infty}\left(V^\pi_i(s) - \widehat{V}^\pi_i(s)\right)\right| \\
&\leq\lambda'\sum_{i'=0}^{i}\gamma^{i'}\max_{s,\pi}\left|{F}(s) - \widehat{F}(s)\right|\leq \lambda'\max_{s,\pi}
\frac{\left|{F}(s) - \widehat{F}(s)\right|}{(1-\gamma)}
\end{align*}







\subsection{Lookup Table Classifier}
If we consider the fear model as a lookup table, and deterministic, then observing each state once is enough to exactly recover the classifier. 



For the stochastic $F$, at time step $N$
\begin{align}\label{eq:hoeffting}
\left|{F}(s) - \widehat{F}(s)\right|\leq \sqrt{\frac{\log{\frac{N}{\delta}}}{N(s)}}
\end{align}
with probability $\delta$ where $N(s)$ is the number visits to a state $s$ at time step $N$. The trajectory produced by algorithm does not produce $i.i.d.$ samples of state. Therefore, for Eq.~\ref{eq:hoeffting} we use Hoeffding's inequality accompanied with union bound over time $N$. In order to have this bound to hold for all the states at once, we need another union bounds over states and all possibly optimal policies $\Pi_\gamma$ under noisy classifier , which requires to replace $\delta\rightarrow \delta/SA\Pi_\gamma$. Let's assume a minimum number of visit $\overline{N}$ to each state,
\begin{align}\label{eq:concnet}
\|V_{F,\gamma}^{\pi^*_{F,\gamma}}-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}\|_\infty \leq \frac{\lambda'}{1-\gamma}\sqrt{\frac{\log{\frac{NSA\Pi_\gamma}{\delta}}}{\overline{N}}}
\end{align}
Finally, adding Eq.~\ref{eq:firstpart} and Eq.~\ref{eq:concnet}, the upper bound on $\mathbb{L}$ is as follows:
\begin{align*}
\mathcal{L}\leq \lambda' \frac{1-\gamma_{eval}}{1-\gamma}\sqrt{\frac{\log{\frac{NSA\Pi_\gamma}{1-\delta}}}{\overline{N}}} + \frac{\gamma_{eval}-\gamma}{1-\gamma}
\end{align*}



\subsection{Classifier from a set of functions}
Let $\mathcal{F}$ denote a set of given binary classifiers and $F\in\mathcal{F}$. In this case, let's assume that we are given a set of $N$ $i.i.d$ samples from the stationary distribution $\omega_{F}^{\pi^*_{\widehat{F},\gamma}}$ . Given a policy $\pi$, the MDP transition process reduces to a Markov chain with transition probability $\mathcal{T}^{\pi}$. Now we rewrite the Eq.~\ref{eq:belman_update} in a matrix format where ${V}^\pi_i,{F}\in\mathbb{R}^{S}$ are vectors of concatenation of $V^\pi_i(s)$ and ${F}(s), ~\forall s\in\mathcal{S}$ respectively.

\begin{align}\label{eq:bellman_vector}
{V}^\pi_i - \widehat{{V}}^\pi_i = \lambda'{{F}} - \lambda'\widehat{{F}} + \gamma \mathcal{T}^{\pi}\left({V}^\pi_{i-1} - \widehat{{V}}^\pi_{i-1}\right)\leq\lambda' \sum_{i'=0}^{i}\left(\gamma\mathcal{T}^{\pi}\right)^{i'}\left({F}-\widehat{{F}}\right)
\end{align}

as $i$ goes to infinity we have 
\begin{align*}
V_{F,\gamma}^{\pi^*_{F,\gamma}}-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}\leq \lambda'\left(\mathbbm{1}-\gamma\mathcal{T}^{\pi}\right)^{-1}\left({F}-\widehat{{F}}\right)
% &= \max_{\pi}	\left|\lim_{i\rightarrow \infty}\left(V^\pi_i(s) - \widehat{V}^\pi_i(s)\right)\right| \\
% &\leq\lambda'\sum_{i'=0}^{i}\gamma^{i'}\max_{s,\pi}\left|{F}(s) - \widehat{F}(s)\right|\leq \lambda'\max_{s,\pi}
% \frac{\left|{F}(s) - \widehat{F}(s)\right|}{(1-\gamma)}
\end{align*}






Using PAC analysis of binary classification in \cite{hanneke2016optimal} a follow up to \cite{vapnik2013nature}, we have 
\begin{align*}
\left|{F} - \widehat{F}\right|^\top \omega_{F}^{\pi^*_{\widehat{F},\gamma}}\leq 3200\frac{\mathcal{VC}(\mathcal{F})+\log{\frac{1}{\delta}}}{N}
\end{align*}
with probability at least $1-\delta$ where $\mathcal{VC}(\mathcal{F})$ is the $\mathcal{VC}$ dimension of the hypothesis class and $|\cdot|$ is entry-wise absolute value. Since $\gamma<1$, then $\alpha_{\max}$, the maximum eigenvalue of $\left(\mathbbm{1}-\gamma\mathcal{T}^{\pi}\right)^{-1}$, is bounded above and we have
\begin{align*}
\|V_{F,\gamma}^{\pi^*_{F,\gamma}}-V_{F,\gamma}^{\pi^*_{\widehat{F},\gamma}}\|_1 \leq 3200\lambda'\alpha_{\max}\frac{\mathcal{VC}(\mathcal{F})+\log{\frac{1}{\delta}}}{N}
\end{align*}
and therefore, 


\begin{align*}
\mathcal{L}\leq 3200\lambda'\alpha_{\max}(1-\gamma_{eval})\frac{\mathcal{VC}(\mathcal{F})+\log{\frac{1}{\delta}}}{N} + \frac{\gamma_{eval}-\gamma}{1-\gamma}
\end{align*}


The remaining part is to solve 
\begin{align*}
\gamma^*=\displaystyle \displaystyle \text{argmin}_{\gamma\leq\gamma_{eval}}\mathcal{L}
\end{align*}
to find the optimal $\gamma$.


The same analysis, up to a slight modification\footnote{Instead of having $V$ as a vector of state values indexed by states, it is a continuous function of states. Furthermore, the Transition kernel is over continuous distribution therefore the same bellman update in Eq.~\ref{eq:bellman_vector} holds.}, holds for the continuous state and action spaces.
 










==> sections/dqn.tex <==
% For context we briefly review deep Q-learning.
Over a series of turns,
an agent interacts with its environment via 
a Markov decision process, or MDP, 
$(\mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma)$.
At each step $t$, an agent observes a state $s\in \mathcal{S}$.
The agent then chooses an action $a\in \mathcal{A}$ according to some policy $\pi$.
In turn, the environment transitions to a new state $s_{t+1} \in \mathcal{S}$ according to transition dynamics $\mathcal{T}(s_{t+1}|s_t,a_t)$ and generates a reward $r_t$ with expectation $\mathcal{R}(s,a)$.
This cycle continues until each episode terminates. 

The goal of an agent is to maximize 
its cumulative discounted return $\sum_{t=0}^T \gamma^t r_{t}$.
Temporal-differences (TD) methods \cite{sutton1988learning} such as Q-learning \cite{watkins1992qlearning} model the Q-function, 
which gives the \emph{optimal} discounted total reward of a state-action pair; the greedy policy w.r.t. the Q-function is optimal \cite{sutton1998reinforcement}.  
Problems of practical interests tend have large state spaces, 
thus the Q-function 
is typically approximated by parametric models such as neural networks.  
 
In deep Q-learning, this is typically accomplished by alternately collecting experiences by acting greedily with respect to $Q(s,a;\theta_Q)$ and updating the parameters $\theta_Q$.
Updates proceed as follows.
For a given experiences $(s_t,a_t,r_t,s_{t+1})$,
we minimize the squared Bellman error: 
\begin{equation}
\mathcal{L} = (Q(s_t,a_t; \theta_Q)-y_t)^2
\end{equation}
for $y_t = r_t + \gamma \cdot \max_{a'} Q(s_{t+1}, a'; \theta_Q)$.
Traditionally, the parameterised $Q(s,a;\theta)$ is trained by stochastic approximation, 
estimating the loss on each experience as it is encountered, yielding the update:
\begin{equation}
\begin{split}
\theta_{t+1} \gets & \theta_t + \alpha (
%r_{t} + \gamma \max_{a'} Q(s_{t+1}, a'; \theta_t) 
y_t - Q(s_t,a_t;\theta_t)) \nabla Q(s_t,a_t;\theta_t)\,.
\end{split}
\end{equation}
Q-learning methods also require an exploration strategy for action selection.  For simplicity, we consider only the $\epsilon$-greedy heuristic.
% However, our techniques apply equally for other exploration strategies such as Thompson Sampling.  For a thorough overview of RL fundamentals, we refer the reader to \citet{sutton1998reinforcement}.
 
A few tricks are often useful to stabilize Q-learning with function approximation.
Of particular relevance to this work is experience replay \cite{lin1992self}: the RL agent maintains a buffer of past experiences, applying TD-learning on randomly selected mini-batches of experience to update the Q-function.  
% This technique has proven effective to make Q-learning more stable and more data-efficient \cite{lin1992self,mnih15human}.



% In practice, the number of states may be intractably large.
% Thus, most practical reinforcement learners approximate the Q function by some parameterized model $Q(s,a;\theta_Q)$,
% among which deep neural networks have risen to prominence.
% Several popular tricks improve deep Q-networks (DQNs) in practice. 
% First, rather than training online, it's common to maintain a buffer of experiences, 
% training on randomly selected mini-batches of experience \cite{lin1992self,mnih15human}. 
% This technique, called \emph{experience replay}, 
% has proven effective and is believed to break up the tight coupling 
% between the observed states and the current policy~\cite{mnih15human}. 
% Second, it's common to periodically cache the parameters $\theta^-$, 
% using these stale parameters to compute the training targets $y_t$. 
% But target freezing confers no benefit on our tasks. 



% We can therefore define the value of an action $a$ in state $s$ as 
% \begin{equation}
% Q^{\pi}(s_t,a_t) = \mathbbm{E}_{\pi}\left[ \sum_{\tau=t}^T \gamma^i r_{\tau} | s_t =s, a_t=a \right]
% \end{equation}
% Given a value function $Q$, the implied policy is to always choose the most valuable action,
% suggesting the recursive formulation
% $$Q(s_t,a_t) = r_t + \gamma \max_{a'} Q(s_{t+1}, a')$$ 

% For a fixed policy, the value function can be iteratively improved
% by approximate value iteration.
% We represent experiences as tuples $(s_t, a_t, r_{t}, s_{t+1})$.
% In Q-learning, we aim to improve the value function (and, in turn, the greedy policy) by minimizing the squared error between the current prediction and the one-step look-ahead prediction
% \begin{equation}
% \mathcal{L}(\theta_t) = 
% \mathbbm{E}_{(s_t,a_t, r_t, s_{t+1}) \sim \rho(\cdot)} \left[
% (y_t - Q(s_t, a_t; \theta_t))^2 
% \right]
% \end{equation}
% for $y_t = r_t + \gamma \max_{a'} Q(s_{t+1}, {a'}; \theta_{t})$ and for $\rho(\cdot)$ denoting the joint distribution of experiences under the current policy.
% Traditionally, the Q-function is trained by stochastic approximation, estimating the loss on each experience as it is encountered, yielding the update:
% \begin{equation}
% \begin{split}
% \theta_{t+1} \gets & \theta_t + \alpha (
% %r_{t} + \gamma \max_{a'} Q(s_{t+1}, a'; \theta_t) 
% y_t - Q(s_t,a_t;\theta_t)) \nabla Q(s_t,a_t;\theta_t).
% \end{split}
% \end{equation}


% We briefly review deep Q-learning for learning to solve a Markov decision process (MDP):
% $M=(\mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma)$.
% At step $t$, the agent observes a state $s_t\in \mathcal{S}$, and chooses an action $a_t\in \mathcal{A}$ according to some policy $\pi$.
% The environment then transitions to a new state $s_{t+1} \in \mathcal{S}$ according to transition dynamics $\mathcal{T}(s_{t+1}|s_t,a_t)$ and generates a reward $r_t$ with expectation $\mathcal{R}(s,a)$.
% This cycle continues until each episode terminates.  The goal is to maximize $\gamma$-discounted total rewards, $\sum_{t=0}^\infty \gamma^t r_t$.

% Temporal-differences (TD) methods~\cite{sutton1988learning} such as Q-learning~\cite{watkins1992qlearning} learn the Q-function, which gives the \emph{optimal} discounted total reward of a state--action pair; the greedy policy w.r.t. the Q-function is optimal~\cite{sutton1998reinforcement}.  Most problems of practical interests have large state spaces, thus the Q-function has to be approximated by parametric models such as neural networks.  A few tricks are often useful to stabilize Q-learning with function approximation.
% Of particular relevance to this work is experience replay~\cite{lin1992self}: the RL agent maintains a buffer of past experiences, applying TD-learning on randomly selected mini-batches of experience to update the Q-function.  This technique has proven effective to make Q-learning more stable and more data-efficient~\cite{lin1992self,mnih15human}.

% %whose greedy policy is optimal.  These methods often use the TD-error, $\delta_t=r_t+\gamma\cdot\max_aQ(s_{t+1},a)-Q(s_t,a_t)$, as the error signals to perform an incremental update to the Q-function.

% \iffalse
% The goal of an agent is to maximize the cumulative discounted return $\sum_{t=0}^T \gamma^t r_{t}$.  In Q-learning, this is accomplished by alternately updating the state-action value function $Q$ and collecting experiences by acting greedily with respect to $Q$.  Specifically, over the course of training, we collect experiences $(s_t,a_t,r_t,s_{t+1})$. To update the $Q$ function, we minimize the squared Bellman error of the current value $Q(s_t,a_t)$, with respect to the temporal difference target  $y_t = r_t + \gamma \cdot \max_{a'} Q(s_{t+1}, a')$.  Q-learning strategies also require an exploration strategy, and for simplicity we consider only the $\epsilon$-greedy heuristic. However, our techniques apply equally for other approaches. For a thorough overview of RL fundamentals, we refer the reader to \cite{sutton1998reinforcement}.
% \fi

% \iffalse
% In practice, the number of states may be intractably large.
% Thus, most practical reinforcement learners approximate the Q function by some parameterized model $Q(s,a;\theta_Q)$,
% among which deep neural networks have risen to prominence.
% Several popular tricks improve deep Q-networks (DQNs) in practice. 
% First, rather than training online, it's common to maintain a buffer of experiences, 
% training on randomly selected mini-batches of experience \cite{lin1992self,mnih15human}. 
% This technique, called \emph{experience replay}, 
% has proven effective and is believed to break up the tight coupling 
% between the observed states and the current policy~\cite{mnih15human}. 
% Second, it's common to periodically cache the parameters $\theta^-$, 
% using these stale parameters to compute the training targets $y_t$. 
% But target freezing confers no benefit on our tasks. 
% \fi

% We can therefore define the value of an action $a$ in state $s$ as 
% \begin{equation}
% Q^{\pi}(s_t,a_t) = \mathbbm{E}_{\pi}\left[ \sum_{\tau=t}^T \gamma^i r_{\tau} | s_t =s, a_t=a \right]
% \end{equation}
% Given a value function $Q$, the implied policy is to always choose the most valuable action,
% suggesting the recursive formulation
% $$Q(s_t,a_t) = r_t + \gamma \max_{a'} Q(s_{t+1}, a')$$ 

% For a fixed policy, the value function can be iteratively improved
% by approximate value iteration.
% We represent experiences as tuples $(s_t, a_t, r_{t}, s_{t+1})$.
% In Q-learning, we aim to improve the value function (and, in turn, the greedy policy) by minimizing the squared error between the current prediction and the one-step look-ahead prediction
% \begin{equation}
% \mathcal{L}(\theta_t) = 
% \mathbbm{E}_{(s_t,a_t, r_t, s_{t+1}) \sim \rho(\cdot)} \left[
% (y_t - Q(s_t, a_t; \theta_t))^2 
% \right]
% \end{equation}
% for $y_t = r_t + \gamma \max_{a'} Q(s_{t+1}, {a'}; \theta_{t})$ and for $\rho(\cdot)$ denoting the joint distribution of experiences under the current policy.
% Traditionally, the Q-function is trained by stochastic approximation, estimating the loss on each experience as it is encountered, yielding the update:
% \begin{equation}
% \begin{split}
% \theta_{t+1} \gets & \theta_t + \alpha (
% %r_{t} + \gamma \max_{a'} Q(s_{t+1}, a'; \theta_t) 
% y_t - Q(s_t,a_t;\theta_t)) \nabla Q(s_t,a_t;\theta_t).
% \end{split}
% \end{equation}









==> sections/safe.tex <==
We now undertake a more formal treatment 
of safe reinforcement learning.  
Precisely what do we mean by \emph{safety}, \emph{catastrophe}, or \emph{danger}? 
The literature offers several notions of safety in reinforcement learning.
\citet{garcia2015comprehensive} provide a comprehensive review of this literature, 
suggesting that existing approaches 
can be divided into two categories.


We see the following problem. The first category of methods acts only on the summary statistics of the return. This can be beneficial because it requires no foreknowledge. But the drawback is that they fundamentally change the objective globally. In reality, we may only wish to avoid a small set of catastrophic states, but might be otherwise happy with maximizing return. On the other hand, processes relying on expert knowledge may presume an unreasonable level of foreknowledge.

In this paper, we propose a new formulation of the safety problem.
We suppose there exists a subset $\mathcal{C} \subset \mathcal{S}$
of avoidable catastrophic states. 
% These states have minimum return, and thus resemble the fatalities of \cite{hans2008safe}.
Additionally, we assume that there exist good policies that never get within a few hops of an avoidable catastrophe.
Just as a child shouldn't run with scissors, 
a self-driving car should never be one split-second decision away from killing a passenger or pedestrian.

Note, this imposes some prior knowledge. 
% In a general, unknown environment, it   that a good policy should get very close to a fatality in order to maximize reward. 
However, the required prior knowledge is minimal. 
We do not ask for foreknowledge over the dynamics in the environment, or of which policies might lead to catastrophes.
All we assume is that catastrophe states are labeled 
as they are encountered.
We might think if this labeling 
as coming from a \emph{catastrophe detector}.
In the case of a self-driving car, 
this might be an impact sensor. 
Even if we can't anticipate all the situations that might lead to an accident, 
we can recognize one when it has already happened 
and take measures to avoid danger zones 
around these states in the future. 


The notion of danger zone suggests some measure of proximity.
Informally, we conceive of \emph{danger} as the likelihood of entering a catastrophe state $c \in \mathcal{C}$ within a short number of steps. 
Note, this probability depends on the policy.
In this paper, we collect the experiences used to train the danger model from the entire training period. So the likelihood here is determined based on the observations of many policies over the course of training. 
Explicitly modeling danger zones can be useful for two reasons. First, it provides a mechanism to avoid oscillating policy learners from repeatedly encountering catastrophe states. Second, reward-shaping to avoid danger zones   can significantly reduce the sample complexity of exploration.


